NODE-ImgNet: a PDE-informed effective and robust model for image denoising

Inspired by the traditional partial differential equation (PDE) approach for image denoising, we propose a novel neural network architecture, referred as NODE-ImgNet, that combines neural ordinary differential equations (NODEs) with convolutional neural network (CNN) blocks. NODE-ImgNet is intrinsically a PDE model, where the dynamic system is learned implicitly without the explicit specification of the PDE. This naturally circumvents the typical issues associated with introducing artifacts during the learning process. By invoking such a NODE structure, which can also be viewed as a continuous variant of a residual network (ResNet) and inherits its advantage in image denoising, our model achieves enhanced accuracy and parameter efficiency. In particular, our model exhibits consistent effectiveness in different scenarios, including denoising gray and color images perturbed by Gaussian noise, as well as real-noisy images, and demonstrates superiority in learning from small image datasets.

==> sec3_IDmodel.tex <==
% \section{NODE Image Denoising model structure}

We assume that for every  noised-ground truth image pair $(h_i(\mathbf{x}), \tilde u_i(\mathbf{x}))_{i=1}^N$,
\yuebox{is the noise from the same source} there exists a vector field  $F({u},t; \mathbf{x})$ such that the ODE solution to the following problem:

 \begin{equation}\label{x-ODE_constant}
 	 \frac{\mathrm{d}{u_{i,\mathbf{x}}}(t)}{\mathrm{d}t} = F({u_{i, \mathbf{x}}},t; \mathbf{x}), \quad {u}(0) = h_i(\mathbf{x}),
 \end{equation} 
 satisfies that
 \[
 u_{i,\mathbf{x}}(T) \equiv \tilde u_i(\mathbf{x}) \quad
 \forall i=1, \cdots, N,  \forall \mathbf{x} \in \Omega.
 \] 
 It is then strightforward to use the XNODE model in \cref{XNODE-model}. We denote the output of the noised image $h_i(\mathbf{x})$ by $ u_{i, \bf{x}}(t):=\text{XNODE}_{\Theta,h_i}(\mathbf{x}, t)$. \yuebox{change notations later}
 
\textcolor{red}{To be added by X.H: Add a figure of the model for the vector field we use. Also, add a suede algorithm.}
%  Note that the assumption using a general vector function $F$ is  more general than using any specific parabolic type PDE model.
% We also note that only the initial condition is needed in the model. Determining the right boundary condition for the PDE related image denoising model has been a challenge task. In this model, we do not require the information of the boundary condition thus eliminate the artificial error caused by using any specific boundary condition.
 

  
 \subsection{Cost functional: $L^p$ norm of the pixel-wise error}
 Our goal is to minimize the following cost functional:
 \[
 		J(\Theta) \approx \dfrac{1}{N}  \| \tilde u_i(\mathbf{x}) - \tilde u_{i, \bf{x}}(T)\|_{L^p(\Omega)}.
 \]

\yuebox{doublecheck the cost above}
